Improving ResBos for the precision needs of the LHC

The resummation calculation (ResBos) is a widely used tool for the simulation of single vector boson production at colliders. In this work, we develop a significant improvement over the ResBos code by increasing the accuracy from NNLL+NLO to N${}^3$LL+NNLO and release the ResBos v2.0 code. Furthermore, we propose a new non-perturbative function that includes information about the rapidity of the system (IFY). The IFY functional form was fitted to data from fixed target experiments, the Tevatron, and the LHC. We find that the non-perturbative function has mild rapidity dependence based on the results of the fit. Finally, we investigate the effects that this increased precision has on the measurement of the $W$ boson by CDF and impacts on future LHC measurements.

==> H2.tex <==
\begin{align}
2C_{q\bar{q}}^{(2)}\left(z\right)&+\delta\left(1-z\right)\left[H_q^{DY(2)}-\frac{3}{4}\left(H_q^{DY(1)}\right)^2+\frac{C_F}{4}\left(\pi^2-8\right)H_q^{DY(1)}\right]\nn\\
&+\frac{1}{2}C_F H_q^{DY(1)}\left(1-z\right)\nn\\
&= \mathcal{H}_{q\bar{q}\leftarrow q\bar{q}}^{DY(2)}\left(z\right)-\frac{C_F^2}{4}\left[\delta\left(1-z\right)\frac{\left(\pi^2-8\right)^2}{4}+\left(\pi^2-10\right)\left(1-z\right)-\left(1+z\right)\ln z\right], \\
C_{qg}^{(2)}\left(z\right)&+\frac{1}{4}H_q^{DY(1)}z\left(1-z\right)=\mathcal{H}_{q\bar{q}\leftarrow qg}^{DY(2)}\left(z\right)\nn\\
&-\frac{C_F}{4}\left[z\ln z + \frac{1}{2}\left(1-z^2\right)+\left(\frac{\pi^2}{4}-4\right) z\left(1-z\right) \right], \\
C_{qq}^{(2)}\left(z\right)&=\mathcal{H}_{q\bar{q}\leftarrow qq}^{DY(2)}\left(z\right), \\
C_{qq'}^{(2)}\left(z\right)&=\mathcal{H}_{q\bar{q}\leftarrow qq'}^{DY(2)}\left(z\right), \\
C_{q\bar{q}'}^{(2)}\left(z\right)&=\mathcal{H}_{q\bar{q}\leftarrow q\bar{q}'},
\end{align}
where the $\mathcal{H}$ coefficients are given by:
\begin{align}
\mathcal{H}^{DY(2)}_{q\bar q\leftarrow q \bar q}(z)&=
C_A C_F 
\bigg\{
\left(\frac{7 \zeta_3}{2}-\frac{101}{27}\right)\left(\frac{1}{1-z}\right)_+ %\text{D0}(z)
+\left(\frac{59 \zeta_3}{18}-\frac{1535}{192}+\frac{215 \pi ^2}{216}-\frac{\pi ^4}{240}\right) \delta(1-z)
\nn\\
&~~~~~~
+\frac{1+z^2}{1-z}
 \bigg(-\frac{\text{Li}_3(1-z)}{2}+\text{Li}_3(z)-\frac{\text{Li}_2(z) \log (z)}{2}
-\frac{1}{2} \text{Li}_2(z) \log (1-z)
\nn\\
&~~~~~~
-\frac{1}{24} \log ^3(z)
-\frac{1}{2} \log ^2(1-z) \log (z)+\frac{1}{12} \pi ^2 \log (1-z)-\frac{\pi ^2}{8}\bigg)
\nn\\
&~~~~~~
+\frac{1}{1-z} \bigg(
-\frac{1}{4} \left(11-3 z^2\right) \zeta_3
-\frac{1}{48} \left(-z^2+12 z+11\right) \log ^2(z)
\nn\\
&~~~~~~
-\frac{1}{36} \left(83 z^2-36 z+29\right) \log (z)+\frac{\pi ^2 z}{4}\bigg)
\nn\\
&~~~~~~
+(1-z) \bigg(\frac{\text{Li}_2(z)}{2}+\frac{1}{2} \log (1-z) \log (z)\bigg)
+\frac{z+100}{27}+\frac{1}{4} z \log (1-z)\bigg\}
\nn\\
&~~~~~~
+C_F n_F \bigg\{\frac{14}{27}\left(\frac{1}{1-z}\right)_+ %\text{D0}(z)
+\frac{1}{864} \left(192 \zeta_3+1143-152 \pi ^2\right) \delta(1-z)
\nn\\
&~~~~~~
+\frac{\left(1+z^2\right)}{72 (1-z)} \log (z) (3 \log (z)+10)+\frac{1}{108} (-19 z-37)\bigg\}
\nn\\
&~~~~~~
+C_F^2 \bigg\{\frac{1}{4} \left(-15 \zeta_3+\frac{511}{16}
-\frac{67 \pi ^2}{12}+\frac{17 \pi ^4}{45}\right) \delta(1-z)
\nn\\&~~~~~~
+\frac{1+z^2}{1-z}
 \bigg(\frac{\text{Li}_3(1-z)}{2}-\frac{5 \text{Li}_3(z)}{2}+\frac{1}{2} \text{Li}_2(z) \log (1-z)
+\frac{3 \text{Li}_2(z) \log (z)}{2}
\nn\\
&~~~~~~
+\frac{3}{4} \log (z) \log ^2(1-z)+\frac{1}{4} \log ^2(z) \log (1-z)-\frac{1}{12} \pi ^2 \log (1-z)+\frac{5 \zeta_3}{2}\bigg)
\nn\\
&~~~~~~
+(1-z) \left(-\text{Li}_2(z)-\frac{3}{2} \log (1-z) \log (z)+\frac{2 \pi ^2}{3}-\frac{29}{4}\right)
+\frac{1}{24} \left(1+z\right) \log ^3(z)
\nn\\
&~~~~~~
+\frac{1}{1-z}\bigg(
\frac{1}{8} \left(-2 z^2+2 z+3\right) \log ^2(z)+\frac{1}{4} \left(17 z^2-13 z+4\right) \log (z)\bigg)
\nn\\
&~~~~~~
-\frac{z}{4}\log (1-z)
\bigg\}
\nn\\
&~~~~~~
+C_F \bigg\{\frac{1}{z}(1-z) \left(2 z^2-z+2\right) \left(\frac{\text{Li}_2(z)}{6}+\frac{1}{6} \log (1-z) \log (z)-\frac{\pi ^2}{36}\right)
\nn\\
&~~~~~~
+\frac{1}{216 z}(1-z) \left(136 z^2-143 z+172\right)-\frac{1}{48} \left(8 z^2+3 z+3\right) \log ^2(z)
\nn\\
&~~~~~~
+\frac{1}{36} \left(32 z^2-30 z+21\right) \log (z)+\frac{1}{24} (1+z) \log ^3(z)
\bigg\}\;,
\end{align}
\begin{align}
{\cal H}^{DY(2)}_{q\bar q\ito q \bar{q}'}(z)&=
C_F \bigg\{
\frac{1}{12 z}(1-z) \left(2 z^2-z+2\right) \bigg(
\text{Li}_2(z)
+\log (1-z) \log (z)
-\frac{\pi^2}{6}
\bigg)
\nn\\
&~~~~~~
+\frac{1}{432 z}(1-z) \left(136 z^2-143 z+172\right)
+\frac{1}{48} (1+z) \log^3(z)
\nn\\&~~~~~~
-\frac{1}{96} \left(8 z^2+3 z+3\right) \log^2(z)
+\frac{1}{72} \left(32 z^2-30 z+21\right) \log (z)
\bigg\}\;,
\label{h2qq}
\end{align}
\begin{align}
{\cal H}^{DY(2)}_{q\bar q\ito q q}(z)&=
C_F\left(C_F-\frac{1}{2}C_A\right)
 \bigg\{ \frac{1+z^2}{1+z}
\bigg(\frac{3 \text{Li}_3(-z)}{2}+\text{Li}_3(z)
+\text{Li}_3\left(\frac{1}{1+z}\right)-\frac{\text{Li}_2(-z) \log (z)}{2}
\nn\\
&~~~~~~
-\frac{\text{Li}_2(z) \log (z)}{2}-\frac{1}{24} \log ^3(z)
-\frac{1}{6} \log ^3(1+z)+\frac{1}{4} \log (1+z) \log ^2(z)
\nn\\
&~~~~~~
+\frac{\pi^2}{12}  \log (1+z)-\frac{3 \zeta_3}{4}\bigg)
+\left(1-z\right) \left(\frac{\text{Li}_2(z)}{2}+\frac{1}{2} \log (1-z) \log (z)+\frac{15}{8}\right)
\nn\\
&~~~~~~
-\frac{1}{2}(1+z) \big(\text{Li}_2(-z)+ \log (z) \log (1+z)\big)
+ \frac{\pi^2}{24}  (z-3)+\frac{1}{8} (11 z+3) \log (z)\bigg\}
\nn\\
&~~~~~~
+C_F \bigg\{\frac{1}{12 z}(1-z) \left(2 z^2-z+2\right) \left(\text{Li}_2(z)+\log (1-z) \log (z)
-\frac{\pi ^2}{6}\right)
\nn\\
&~~~~~~
+\frac{1}{432 z}(1-z) \left(136 z^2-143 z+172\right)-\frac{1}{96} \left(8 z^2+3 z+3\right) \log ^2(z)
\nn\\
&~~~~~~
+\frac{1}{72} \left(32 z^2-30 z+21\right) \log (z)+\frac{1}{48} (1+z) \log ^3(z)\bigg\}
\;,
\end{align}
\begin{align}
\label{h2qqp}
\mathcal{H}^{DY(2)}_{q\bar q\ito q q'}(z)=\mathcal{ H}^{DY(2)}_{q\bar q\ito q \bar{q}'}(z)\;,
\end{align}
\begin{align}
\label{h2qg}
{\cal H}^{DY(2)}_{q \bar q\ito qg}(z)
&=
C_A \bigg\{-\frac{1}{12 z}(1-z) \left(11 z^2-z+2\right) \text{Li}_2(1-z)
\nn\\
&~~~~~~
+\left(2 z^2-2 z+1\right) \bigg(\frac{\text{Li}_3(1-z)}{8}
-\frac{1}{8} \text{Li}_2(1-z) \log (1-z)+\frac{1}{48} \log^3(1-z)\bigg)
\nn\\
&~~~~~~
+\left(2 z^2+2 z+1\right) \bigg(\frac{3 \text{Li}_3(-z)}{8}
+\frac{\text{Li}_3\left(\frac{1}{1+z}\right)}{4}-\frac{\text{Li}_2(-z) \log(z)}{8}
-\frac{1}{24} \log^3(1+z)
\nn\\
&~~~~~~
+\frac{1}{16} \log^2(z) \log (1+z)
+\frac{1}{48} \pi^2 \log (1+z)\bigg)
+\frac{1}{4} z (1+z) \text{Li}_2(-z)+z \text{Li}_3(z)
\nn\\
&~~~~~~
-\frac{1}{2} z \text{Li}_2(1-z) \log(z)-z \text{Li}_2(z) \log(z)
-\frac{3}{8} \left(2 z^2+1\right) \zeta_3-\frac{149 z^2}{216}
\nn\\
&~~~~~~
-\frac{1}{96} \left(44 z^2-12 z+3\right) \log^2(z)
+\frac{1}{72} \left(68 z^2+6 \pi^2 z-30 z+21\right) \log(z)
\nn\\
&~~~~~~
+\frac{\pi^2 z}{24}+\frac{43 z}{48}
+\frac{43}{108 z}+\frac{1}{48} (2 z+1) \log^3(z)
-\frac{1}{2} z \log (1-z) \log^2(z)
\nn\\
&~~~~~~
-\frac{1}{8} (1-z) z \log^2(1-z)
+\frac{1}{4} z (1+z) \log (1+z) \log(z)
\nn\\
&~~~~~~
+\frac{1}{16} (3-4 z) z \log (1-z)-\frac{35}{48}\bigg\}
\nn\\
&~~~~~~
+C_F \bigg\{\left(2 z^2-2 z+1\right) 
\bigg(\zeta_3-\frac{\text{Li}_3(1-z)}{8}
-\frac{\text{Li}_3(z)}{8}+\frac{1}{8} \text{Li}_2(1-z) \log (1-z)
\nn\\
&~~~~~~
+\frac{\text{Li}_2(z) \log(z)}{8}-\frac{1}{48} \log^3(1-z)
+\frac{1}{16} \log(z) \log^2(1-z)
\nn\\
&~~~~~~
+\frac{1}{16} \log^2(z) \log (1-z)
\bigg)
\nn\\
&~~~~~~
-\frac{3 z^2}{8}-\frac{1}{96} \left(4 z^2-2 z+1\right) \log^3(z)
+\frac{1}{64} \left(-8 z^2+12 z+1\right) \log^2(z)
\nn\\
&~~~~~~
+\frac{1}{32} \left(-8 z^2+23 z+8\right) \log(z)+\frac{5}{24} \pi^2 (1-z) z
+\frac{11 z}{32}+\frac{1}{8} (1-z) z \log^2(1-z)
\nn\\
&~~~~~~
-\frac{1}{4} (1-z) z \log (1-z) \log(z)
-\frac{1}{16} (3-4 z) z \log (1-z)-\frac{9}{32}\bigg\}\;,
\end{align}
\begin{align}
\label{h2gg}
\mathcal{H}^{DY(2)}_{q\bar q\ito gg}(z)&=
-\,\frac{z}{2}\,\left(\,1-z+\frac{1}{2}\,(1+z)\,\log (z)\, \right)\;,
\end{align}
